Explicit Approximations of the Gaussian Kernel

We investigate training and using Gaussian kernel SVMs by approximating the kernel with an explicit finite- dimensional polynomial feature representation based on the Taylor expansion of the exponential. Although not as efficient as the recently-proposed random Fourier features [Rahimi and Recht, 2007] in terms of the number of features, we show how this polynomial representation can provide a better approximation in terms of the computational cost involved. This makes our "Taylor features" especially attractive for use on very large data sets, in conjunction with online or stochastic training.

==> Makefile <==
PDFLATEX = pdflatex -file-line-error -halt-on-error
LATEX = latex

FILES = \
	main.tex \
	macros.tex \
	abstract.tex \
	sec_comparison.tex \
	sec_conclusion.tex \
	sec_experiments.tex \
	sec_introduction.tex \
	sec_preliminaries.tex \
	sec_random_features.tex \
	sec_taylor_features.tex \
	sec_polynomial.tex \
	figures/fig_cov1.tex \
	figures/fig_experiments.tex \
	figures/tab_datasets.tex \
	figures/tab_kernel_errors.tex \
	figures/tab_polynomial.tex \
	main.bib

.PHONY : all
all: main.pdf

main.pdf: $(FILES)
	$(PDFLATEX) main.tex
	bibtex main
	$(PDFLATEX) main.tex
	$(PDFLATEX) main.tex
	pdftops main.pdf
	ps2pdf14 -dPDFSETTINGS=/prepress main.ps

.PHONY: clean
clean:
	rm -f main.aux main.bbl main.blg main.log main.out main.tpm
	rm -f main.dvi main.ps main.pdf


==> app_hermite.tex <==
\section{Proof of theorem \ref{thm:hermite}}\label{app:hermite}

The Hermite functions $\psi_{k}$, which are eigenfunctions of the Fourier
transform, are defined in terms of Hermite polynomials $H_{k}$ as:
%
(%\url{http://en.wikipedia.org/wiki/Hermite_polynomials})
%
%
\begin{align*}
%
\psi_{k}\left(x\right) & =
	\frac{1}{\sqrt{\left(k!\right)2^{k}\sqrt{\pi}}}e^{-\frac{1}{2}x^{2}}H_{k}\left(x\right)\\
H_{0}\left(x\right) & = 1\\
H_{1}\left(x\right) & = 2x\\
H_{k+1}\left(x\right) & = 2xH_{k}\left(x\right)-2kH_{k-1}\left(x\right)
%
\end{align*}
%
One of the most important properties of the Hermite functions, and the one upon
which we will rely here, is that they are the eigenfunctions of the Fourier
transform. We will begin with a lemma which will permit us to expand the
Gaussian kernel for one-dimensional data in terms of Hermite functions
multiplied by some additional exponential scaling:

\begin{lemma}\label{lem:hermite_eigenfunctions}
%
Define
$f\left(x,y\right)=e^{-\frac{1}{2\sqrt{3}}x^{2}}e^{-\frac{1}{2\sqrt{3}}\left(x-y\right)^{2}}e^{-\frac{1}{2\sqrt{3}}y^{2}}$.
The eigenfunctions of $f$--the orthonormal $\varphi$ which maximize:
%
\begin{align*}
%
\left\langle \varphi\mid f\mid\varphi\right\rangle & =
	\int\int\varphi\left(x\right)f\left(x,y\right)\varphi\left(y\right)dxdy
%
\end{align*}
%
are proportional to the Hermite functions: $\varphi\propto\psi_{k}$.
%
\end{lemma}
%
\begin{proof}
%
Writing $\varphi$ in terms of its Fourier transform:
%
\begin{align*}
%
\varphi\left(x\right) & \propto 
	\int e^{ix\hat{x}}\hat{\varphi}\left(\hat{x}\right)d\hat{x}
%
\end{align*}
%
gives that:
%
\begin{align*}
%
\int\varphi\left(x\right)e^{-\frac{1}{2\sqrt{3}}x^{2}}e^{-\frac{1}{2\sqrt{3}}\left(x-y\right)^{2}}dx & \propto
	\int\int e^{ix\hat{x}}\hat{\varphi}\left(\hat{x}\right)e^{-\frac{1}{2\sqrt{3}}x^{2}}e^{-\frac{1}{2\sqrt{3}}\left(x-y\right)^{2}}dxd\hat{x}\\
& \propto
	\int\int e^{ix\hat{x}}\hat{\varphi}\left(\hat{x}\right)e^{-\frac{1}{\sqrt{3}}\left(x-\frac{1}{2}y\right)^{2}}e^{-\frac{1}{4\sqrt{3}}y^{2}}dxd\hat{x}\\
& \propto
	\int\hat{\varphi}\left(\hat{x}\right)e^{-\frac{\sqrt{3}}{4}\hat{x}^{2}}e^{i\frac{y\hat{x}}{2}}e^{-\frac{1}{4\sqrt{3}}y^{2}}d\hat{x}
%
\end{align*}
%
and:
%
\begin{align*}
%
\int\varphi\left(y\right)e^{i\frac{y\hat{x}}{2}}e^{-\frac{1}{4\sqrt{3}}y^{2}}e^{-\frac{1}{2\sqrt{3}}y^{2}}dy & \propto
	\int\int e^{iy\hat{y}}\hat{\varphi}\left(\hat{y}\right)e^{i\frac{y\hat{x}}{2}}e^{-\frac{1}{4\sqrt{3}}y^{2}}e^{-\frac{1}{2\sqrt{3}}y^{2}}dyd\hat{y}\\
& \propto
	\int\hat{\varphi}\left(\hat{y}\right)e^{-\frac{1}{\sqrt{3}}\left(\hat{y}+\frac{1}{2}\hat{x}\right)^{2}}d\hat{y}
%
\end{align*}
%
so:
%
\begin{align*}
%
\left\langle \varphi\mid f\mid\varphi\right\rangle & \propto
	\int\int\hat{\varphi}\left(\hat{x}\right)e^{-\frac{\sqrt{3}}{4}\hat{x}^{2}}e^{-\frac{1}{\sqrt{3}}\left(\hat{y}+\frac{1}{2}\hat{x}\right)^{2}}\hat{\varphi}\left(\hat{y}\right)d\hat{x}d\hat{y}\\
& \propto
	\int\int\overline{\hat{\varphi}\left(\hat{x}\right)}e^{-\frac{\sqrt{3}}{4}\hat{x}^{2}}e^{-\frac{1}{\sqrt{3}}\left(\hat{y}-\frac{1}{2}\hat{x}\right)^{2}}\hat{\varphi}\left(\hat{y}\right)d\hat{x}d\hat{y}\\
& \propto
	\int\int\overline{\hat{\varphi}\left(\hat{x}\right)}e^{-\frac{1}{2\sqrt{3}}\hat{x}^{2}}e^{-\frac{1}{2\sqrt{3}}\left(\hat{x}-\hat{y}\right)^{2}}e^{-\frac{1}{2\sqrt{3}}\hat{y}^{2}}\hat{\varphi}\left(\hat{y}\right)d\hat{x}d\hat{y}\\
& \propto
	\left\langle \hat{\varphi}\mid f\mid\hat{\varphi}\right\rangle
%
\end{align*}
%
By Parseval's theorem, $\left\Vert \varphi\right\Vert =\left\Vert
\hat{\varphi}\right\Vert$ and $\left\langle
\varphi_{j}\mid\varphi_{k}\right\rangle =\left\langle
\hat{\varphi}_{j}\mid\hat{\varphi}_{k}\right\rangle$.  Hence, the orthonormal
sequence of $\varphi$ which maximizes $\left\langle \varphi\mid
f\mid\varphi\right\rangle$ will be precisely the same as the orthonormal
sequence which maximizes $\left\langle \hat{\varphi}\mid
f\mid\hat{\varphi}\right\rangle$, implying that $\varphi=\hat{\varphi}$ for all
eigenfunctions of $f$, so $\varphi\propto\psi_{k}$.
%
\end{proof}

Define the {}``outer product'' of two Hermite functions
$\psi_{k}\left(x,y\right)=\psi_{k}\left(x\right)\psi_{k}\left(y\right)$, and
note that these functions are orthonormal:
%
\begin{align*}
%
\int\int\psi_{k}\left(x,y\right)\psi_{k'}\left(x,y\right)dxdy & =
	\left(\int\psi_{k}\left(x\right)\psi_{k'}\left(x\right)dx\right)^{2}\\
& = \delta_{k,k'}
%
\end{align*}
%
These functions do not form a complete set, but lemma
\ref{lem:hermite_eigenfunctions}, which implies that $f$ may be represented as
a linear combination of these functions, gives that:
%
\begin{align*}
%
f\left(x,y\right) & = \sum_{k}c_{k}\psi_{k}\left(x,y\right)\\
c_{k} & = \int\int f\left(x,y\right)\psi_{k}\left(x,y\right)dxdy
%
\end{align*}
%
so that in particular:
%
\begin{align*}
%
e^{-\frac{1}{2\sqrt{3}}\left(x-y\right)^{2}} & =
	\sum_{k=0}^{\infty}c_{k}\left(e^{\frac{1}{2\sqrt{3}}x^{2}}\psi_{k}\left(x\right)\right)\left(e^{\frac{1}{2\sqrt{3}}y^{2}}\psi_{k}\left(y\right)\right)
%
\end{align*}
%
A substitution gives that:
%
\begin{align*}
%
e^{-\frac{1}{2}\left(x-y\right)^{2}} & =
	\sum_{k=0}^{\infty}c_{k}\left(e^{\frac{1}{2}x^{2}}\psi_{k}\left(\sqrt[4]{3}x\right)\right)\left(e^{\frac{1}{2\sqrt{3}}y^{2}}\psi_{k}\left(\sqrt[4]{3}y\right)\right)
%
\end{align*}
%
which, combined with the fact that, as eigenvalues of a positive definite
operator, the $c_{k}$s are positive, permits us to state a corollary:

\begin{corollary}\label{cor:hermite_expansion}
%
If $K\left(x,y\right)=e^{-\frac{1}{2}\left(x-y\right)^{2}}$ and
$\phi_{k}\left(x\right)=\sqrt{c_{k}}e^{\frac{1}{2}x^{2}}\psi_{k}\left(\sqrt[4]{3}x\right)$,
then:
%
\begin{align*}
%
K\left(x,y\right) & =
	\left\langle \phi\left(x\right)\mid\phi\left(y\right)\right\rangle
%
\end{align*}
%
\end{corollary}

The following lemma shows that these functions form the (uncentered) kernel PCA
basis for the Gaussian kernel, for Gaussian-distributed data:

\begin{lemma}\label{lem:hermite_kpca}
%
If $x\sim\mathcal{N}\left(0,\frac{1}{2}\right)$ and
$\phi_{k}\left(x\right)=\sqrt{c_{k}}e^{\frac{1}{2}x^{2}}\psi_{k}\left(\sqrt[4]{3}x\right)$,
then
$E_{x}\left[\phi_{j}\left(x\right)\phi_{k}\left(x\right)\right]=\delta_{j,k}\left(\pi\sqrt{3}\right)^{-\frac{1}{2}}c_{k}$.
%
\end{lemma}
%
\begin{proof}
%
Writing the expectation as an integral:
%
\begin{align*}
%
E_{x}\left[\phi_{j}\left(x\right)\phi_{k}\left(x\right)\right] & =
	\sqrt{c_{j}c_{k}}\int e^{x^{2}}\psi_{j}\left(\sqrt[4]{3}x\right)\psi_{k}\left(\sqrt[4]{3}x\right)dP\left(x\right)\\
& = \sqrt{\frac{c_{j}c_{k}}{\pi}}\int\psi_{j}\left(\sqrt[4]{3}x\right)\psi_{k}\left(\sqrt[4]{3}x\right)dx\\
& = \delta_{j,k}\sqrt{\frac{c_{j}c_{k}}{\pi\sqrt{3}}}
%
\end{align*}
%
where above we used the orthonormality of the Hermite functions to evaluate the
integral.
%
\end{proof}

We may now generalize these results to the multidimensional case.  Suppose that
$x\in\mathbb{R}^{d}$. Then by corollary \ref{cor:hermite_expansion}:
%
\begin{align*}
%
e^{-\frac{1}{2}\left\Vert x-y\right\Vert _{2}^{2}} & =
	\prod_{j=1}^{d}e^{-\frac{1}{2}\left(x_{j}-y_{j}\right)^{2}}\\
& = \prod_{i=1}^{d}\sum_{k=0}^{\infty}\left(\sqrt{c_{k}}e^{\frac{1}{2}x_{i}^{2}}\psi_{k}\left(\sqrt[4]{3}x_{i}\right)\right)\left(\sqrt{c_{k}}e^{\frac{1}{2\sqrt{3}}y_{i}^{2}}\psi_{k}\left(\sqrt[4]{3}y_{i}\right)\right)\\
& = \sum_{k\in\mathbb{N}^{d}}\left(e^{\frac{1}{2}\left\Vert x\right\Vert
	_{2}^{2}}\prod_{i=1}^{d}\sqrt{c_{k_{i}}}\psi_{k_{i}}\left(\sqrt[4]{3}x_{i}\right)\right)\left(e^{\frac{1}{2}\left\Vert
	y\right\Vert
	_{2}^{2}}\prod_{i=1}^{d}\sqrt{c_{k_{i}}}\psi_{k_{i}}\left(\sqrt[4]{3}y_{i}\right)\right)
%
\end{align*}
%
Implying that if we define $\phi_{k}\left(x\right)=e^{\frac{1}{2}\left\Vert
x\right\Vert
_{2}^{2}}\prod_{i=1}^{d}\sqrt{c_{k_{i}}}\psi_{k_{i}}\left(\sqrt[4]{3}x_{i}\right)$
for $k\in\mathbb{N}^{d}$, then $K\left(x,y\right)=\left\langle
\phi\left(x\right)\mid\phi\left(y\right)\right\rangle$.  Furthermore, if we
suppose that $x\sim\mathcal{N}\left(0,\frac{1}{2}I\right)$ then the
following expectation decomposes into a product of expectations over the
marginals in each dimension, allowing us to apply lemma \ref{lem:hermite_kpca}
to show that these features are projections onto the uncentered kernel PCA
basis:
%
\begin{align*}
%
E_{x}\left[\phi_{j}\left(x\right)\phi_{k}\left(x\right)\right] & =
	\int\prod_{i=1}^{d}\sqrt{c_{j_{i}}c_{k_{i}}}e^{x_{i}^{2}}\psi_{k_{i}}\left(\sqrt[4]{3}x_{i}\right)\psi_{j_{i}}\left(\sqrt[4]{3}x_{i}\right)dP\left(x\right)\\
& = \prod_{i=1}^{d}\delta_{j_{i},k_{i}}\left(\pi\sqrt{3}\right)^{-\frac{1}{2}}c_{k_{i}}\\
& = \delta_{j,k}\left(\pi\sqrt{3}\right)^{-\frac{d}{2}}\prod_{i=1}^{d}c_{k_{i}}
%
\end{align*}
%
which in particular gives that, because $K\left(x,x\right)=1$, if we sum only
over the indices $k\in\mathcal{K}$:
%
\begin{align*}
%
E_{x}\left[K\left(x,x\right)-\sum_{k\in\mathcal{K}}\phi_{k}\left(x\right)\phi_{k}\left(x\right)\right]
& = 1-\left(\pi\sqrt{3}\right)^{-\frac{d}{2}}\sum_{k\in\mathcal{K}}\prod_{i=1}^{d}c_{k_{i}}
%
\end{align*}


==> figures/fig_timit3.tex <==
\begin{figure*}[tb]

\noindent \begin{centering}
\begin{tabular}{ @{} L @{} S @{} L @{} S @{} S @{} }

\multicolumn{5}{c}{TIMIT} \\

\rotatebox{90}{\scriptsize{Primal objective}} &
\includegraphics[width=0.29\textwidth]{plots/timit3_primal} &
\includegraphics[width=0.29\textwidth]{plots/timit3_primal_features} &
\rotatebox{90}{\scriptsize{Average $\left\vert K - \tilde{K} \right\vert$}} &
\includegraphics[width=0.29\textwidth]{plots/timit3_kernel_cost} \\[-3pt]
& \scriptsize{Computational cost} & \scriptsize{\# features} & & \scriptsize{Computational cost} \\

\rotatebox{90}{\scriptsize{Testing classification error}} &
\includegraphics[width=0.29\textwidth]{plots/timit3_classification} &
\includegraphics[width=0.29\textwidth]{plots/timit3_sigma_test} &
\rotatebox{90}{\scriptsize{Average $\left\vert K - \tilde{K} \right\vert$}} &
\includegraphics[width=0.29\textwidth]{plots/timit3_kernel_features} \\[-3pt]
& \scriptsize{Computational cost} & \scriptsize{$\sigma$} & & \scriptsize{\# features} \\

\end{tabular}
\end{centering}

\caption{
%
Left column: same as Figure \ref{fig:experiments}. Top middle: primal objective
as a function of the total number of features (in log scale). Bottom middle:
test error as a function of the Gaussian kernel parameter $\sigma$, for Taylor
and random Fourier expansions of the same computational cost. Right column:
average value of the approximation error $| K\left( x, x' \right) -
\tilde{K}\left( x, x' \right) |$ over 100000 randomly chosen pairs of training
vectors, in terms of both computational cost and total number of features.
%
}

\label{fig:timit3}

\end{figure*}


==> figures/tab_kernel_errors.tex <==
\begin{table*}[tb]

\caption{
%
Average value of $\left\vert K\left( x, y \right) - \tilde{K}\left( x, y
\right) \right\vert$ over $100000$ pairs randomly sampled from each dataset, as
well as the average computational cost (in units of floating point operations)
of calculating the feature vector $\tilde\phi\left( x \right)$.  All quantities
are reported to three significant digits.
%
}

\begin{centering}

\begin{tabular}{||c|c|c||c|c||c|c||c|c||c|c||}
\multicolumn{3}{||c||}{} & \multicolumn{8}{c||}{Dataset}\\
\multicolumn{3}{||c||}{Method} & \multicolumn{2}{c||}{Adult} & \multicolumn{2}{c||}{Cov1} & \multicolumn{2}{c||}{MNIST} & \multicolumn{2}{c||}{TIMIT}\\
Type & $D$ & $r$ & Cost & Error & Cost & Error & Cost & Error & Cost & Error\\
\hline
\hline
%Fourier & $16$ &  & $254$ & $0.105$ & $224$ & $0.141$ & $2430$ & $0.137$ & $656$ & $0.137$\\
%\hline
%Fourier & $32$ &  & $508$ & $0.0787$ & $448$ & $0.100$ & $4860$ & $0.0950$ & $1310$ & $0.0961$\\
%\hline
%Fourier & $64$ &  & $1020$ & $0.0540$ & $896$ & $0.0706$ & $9720$ & $0.0690$ & $2620$ & $0.0669$\\
%\hline
%Fourier & $128$ &  & $2030$ & $0.0394$ & $1790$ & $0.0506$ & $19400$ & $0.0505$ & $5250$ & $0.0480$\\
%\hline
Fourier & $256$ &  & $4060$ & $0.0276$ & $3580$ & $0.0360$ & $38900$ & $0.0368$ & $10500$ & $0.0350$\\
\hline
Fourier & $512$ &  & $8120$ & $0.0195$ & $7170$ & $0.0263$ & $77800$ & $0.0277$ & $21000$ & $0.0239$\\
\hline
Fourier & $1024$ &  & $16200$ & $0.0160$ & $14300$ & $0.0191$ & $156000$ & $0.0232$ & $42000$ & $0.0171$\\
\hline
Fourier & $2048$ &  & $32500$ & $0.0129$ & $28700$ & $0.0140$ & $311000$ & $0.0195$ & $84000$ & $0.0119$\\
\hline
Fourier & $4096$ &  & $65000$ & $0.00961$ & $57300$ & $0.0107$ & $622000$ & $0.0164$ & $168000$ & $0.00853$\\
\hline
Taylor &  & $2$ & $118$ & $0.0203$ & $91$ & $0.00924$ & $12300$ & $0.0403$ & $820$ & $0.00374$\\
\hline
Taylor &  & $3$ & $666$ & $0.00760$ & $455$ & $0.00817$ & $716000$ & $0.0255$ & $11500$ & $0.000942$\\
\hline
Taylor &  & $4$ & $2980$ & $0.00512$ & $1820$ & $0.00691$ &  &  & $123000$ & $0.000215$\\
\hline
Taylor &  & $5$ & $11300$ & $0.00468$ & $6190$ & $0.00617$ &  &  & $1090000$ & $0.0000484$\\
\hline
\end{tabular}

\end{centering}

\label{tab:kernel_errors}

\end{table*}

